Sovereign: User-Controlled Smart Homes

Recent years have witnessed the rapid deployment of smart homes; most of them are controlled by remote servers in the cloud. Such designs raise security and privacy concerns for end users. In this paper, we describe the design of Sovereign, a home IoT system framework that provides end users complete control of their home IoT systems. Sovereign lets home IoT devices and applications communicate via application-named data and secures data directly. This enables direct, secure, one-to-one and one-to-many device-to-device communication over wireless broadcast media. Sovereign utilizes semantic names to construct usable security solutions. We implement Sovereign as a publish-subscribe-based development platform together with a prototype home IoT controller. Our preliminary evaluation shows that Sovereign provides a systematic, easy-to-use solution to user-controlled, self-contained smart homes running on existing IoT hardware without imposing noticeable overhead.

==> sections/security.tex <==
%\section{Securing \sysname Home System}
%\label{sec:security}
%
%\sysname secures the whole system with a data-centric solution, where \first data instead of channels is secured and \second security policies defined by users are enforced at each system participant instead at centralized cloud.
%
%In \sysname, the control flow starts from users' configuration and ends with security rules distributed to system participants.
%These rules define how cryptographic materials are used in securing and verifying packets.
%The security rules will then be enforced in data flow, \ie content delivery and service invocation.

\mypara{Participant Bootstrapping}
%%Before any security rules can be made or executed, the system must be aware of
\sysname must know the identities of all system participants, so that the defined security rules can be made based on, and delivered to, the corresponding participants.
To integrate a new device or application into the system, the first step is participant bootstrapping, \ie installing into the new participant the local trust anchor and identity names with corresponding cryptographic material and rules.

The controller bootstraps a new device through direct device-to-device connectivity (\eg Bluetooth).
In this process, the controller listens on a specific name, \eg \name{/signon}, and the new device will periodically broadcast requests to that name.
To establish mutual trust between the device and the controller, the user will need to perform certain out-of-band operations such as QR code scanning.

After the pairing, the following cryptographic material is exchanged.
\begin{enumerate} [leftmargin=*, itemsep=1pt, topsep=1pt]
	\item The trust anchor certificate is installed into the device, enabling it to authenticate data published by the controller or other system members.

	\item The controller determines the identity name by following defined naming convention as shown in Table~\ref{tab:naming_convention}, with some name components taking input from the user (\eg selecting a room if applicable, or assigning a customized id).
	\item The controller certifies the device and issues certificates for the device's identity keys, enabling it to publish content and commands that can be authenticated by other system members.

	\item Necessary encryption and decryption keys are also obtained by the device to encrypt data it generates, and to access data the device is authorized to read.
	This step might also require certain authorization from a higher layer (\eg end users).

	\item Name-based rules that will be used by the participant.

	\item Other information, including a secret shared among the participant and the controller for later key renewal processes (\ie encrypt the new key with the shared secret so that only the right participant can decrypt it).
\end{enumerate}
A specific construction of device security bootstrapping that can be used by \sysname is described in~\cite{ssp-li}.

Bootstrapping \sysname applications follows steps similar to the above.
Note that applications can either run locally (\eg software downloaded to the home hub) or remotely (\eg cloud services).
When bootstrapping a remote application, NDN tunnels can be built over IP and the trust can be established via Single Sign-on (SSO) or by other means.

\mypara{Data Authentication}
In \sysname, all content Data packets are signed by their producers and all service invocation command Data packets are signed by the requesters to ensure data integrity and authenticity.
To enforce strict control, \sysname utilizes name-based rules to precisely define the relation between signer's identity name and the name of the data being signed.
For example, a temperature sensor's key cannot be used to sign the status content of a door lock.
Utilizing the three-tuple, this can be represented as follows.
\begin{center}
\ndnname{</alice-home/TEMP, produce, /alice-home/TEMP/CONTENT>}
\end{center}
As shown in the rule, \ndnname{/alice-home/TEMP} is the shared prefix of all home temperature sensors, and \ndnname{/alice-home/TEMP/CONTENT} is the common prefix of content produced under the temperature service.

With such security rules, \sysname participants can verify each received content to ensure not only it is generated by a legitimate participant but also this participant is authorized to produce such piece of content.
The security rules also restrict which named participant is allowed to issue what requests to invoke executables for access control, as described next.

\mypara{Access Control}
In \sysname, the access control policies are also expressed by name-based rule <object, access, subject>, based on \first both system participants and resources are named and \second identity names are cryptographically bound to participants.
After the rules are generated by the controller, they are installed in the participants that are involved in the rule.
For example, a rule as follows indicates that all the automation applications running on the hub can invoke the executables whose names match the specified regular expression (\ndnname{<>*} can match zero or more name components).
\begin{center}
\ndnname{</alice-home/AUTOMATION/hub, access, /alice-home/LOCK/<>*/CMD>}
\end{center}
Such a rule will be packed into rule NDN Data packets following the naming conventions and will be fetched, verified, and loaded by all home hub applications and lock service providers at home.

Regarding access control of service invocation, when sending out a request to invoke an executable of a service, the sender will check whether there is a matching rule.
If so, the participant will use its own private key to sign the request; otherwise, the request will fail.
On the receiver side, a participant will \first verify the signature is from a valid participant and \second check whether there is an available rule for the signer to access the corresponding executable.

As for content access control, \sysname provides content access control by encryption.
Regarding content fetching, the system allows every participant to fetch any piece of content using NDN Interest packets carrying the content name.
However, this does not mean every participant can access any piece of content because all content is encrypted by its producer using proper encryption key obtained from the controller.
To decrypt the content, a participant will need to obtain the decryption key from the controller.
If there is no corresponding rule,

As a consequence, the access to content is equivalent to access to corresponding decryption key delivery service, which follows the aforementioned service invocation access control process.
To be more specific, name-based rules will be used to restrict which participants can access which keys.
For example, ``bedroom air conditioners can read the temperature'' can be written as follows.
\begin{center}
\ndnname{</alice-home/AirCon/bedroom, access, /alice-home/TEMP/DKEY>}
\end{center}
The subject name \ndnname{/alice-home/TEMP/DKEY} represents the decryption key for content produced under the temperature service.

Usually the encryption and decryption key are obtained during the participant bootstrapping process.
However, when keys needs to be renewed or changed (\eg for access right revocation purpose), a participant needs to securely get new keys from the controller.
In \sysname, the participant can fetch new keys with Interest packets constructed with the naming convention and decrypt the new keys with the shared secret between the participant and controller.
The keys can be saved at home storage service so that the keys remain available even when the controller is down

In our prototype implementation, we select service as the access granularity and the symmetric AES encryption as the encryption mechanism.
However, our framework can be easily adapted to other access granularity and encryption schemes.
For example, to support per-service per-room level access control and IoT attribute-based encryption scheme proposed by \fillme~\cite{bibid}, the encryption/decryption key can be named like \ndnname{/alice-home/<service>/<room>/EKEY, .../DKEY}. Correspondingly, the controller will need to prepare proper attributes and policies for data of each service and room combination.



\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\textwidth]{figures/name-tree}
	\vspace{-0.4cm}
	\caption{Fine-grained Service Access Control Policies}
	\vspace{-0.3cm}
	\label{fig:trust_name_tree}
\end{figure}


\subsection{Fine Granularity in Security Rules}

\zhiyi{Merge this into the previous sections}

By properly define rules with names of different level of precision, the security rules for data authentication and access control can be fine-grained.
To be more specific, when specifying the object name or a subject name in a rule, a prefix or name with regular expression can be used to represent a set of participants or resources (\ie content and invocable services)

For example, Figure~\ref{fig:trust_name_tree} shows two name trees where the left one is the identity name tree for system participants and the right tree represents the invocable services (under the prefix \name{/alice-home/LOCK/CMD}) and content (under the prefix \name{/alice-home/LOCK/CONTENT}) under the lock service.
Each arrow in the figure represent a security rule.

Policy \ding{202} defines that any participant in the system (all participants' names are under the prefix \name{/alice-home}) can invoke any executable under the LOCK service.
The name \name{/alice-home/LOCK/CMD} is the common prefix of all executables under the LOCK service.
Policies \ding{203}, \ding{204}, and \ding{205} are of three levels of granularity.
They define the hub application ``app-1'' can command all locks in the bed room (room wide), the ``front'' lock (device wide), and issue only the lock command to the ``front'' lock (command wide), respectively.
 Policy \ding{206} requires that only the lock called ``front'' can produce the state of itself.

\sysname also supports the use of wildcard in security rules.
For example, a rule that allows a participant to access prefix \name{/alice-home/<>/CMD/livingroom}
means the participant can command executables under any service in the living room, where an empty \name{<>} can match any single name component.
